A proposed solution for analysis management in high energy physics

This paper presents an architecture for the analysis management in high energy physics experiments. Some new concepts on data analysis are introduced. A protocol for organizing and operating an analysis is raised. A toolkit following this architecture is developed, which provides a solution of analysis management with both flexibility and reproducibility. A foreseen development of this toolkit is discussed.

==> HeaderFiles.tex <==
\section{Header Files}
In general, every .cc file should have an associated .h file. There are some common exceptions, such as unittests and small .cc files containing just a main() function.

Correct use of header files can make a huge difference to the readability, size and performance of your code.

The following rules will guide you through the various pitfalls of using header files.

\subsection{Self-contained Headers}

Header files should be self-contained (compile on their own) and end in .h. Non-header files that are meant for inclusion should end in .inc and be used sparingly.

All header files should be self-contained. Users and refactoring tools should not have to adhere to special conditions to include the header. Specifically, a header should have header guards and include all other headers it needs.

Prefer placing the definitions for template and inline functions in the same file as their declarations. The definitions of these constructs must be included into every .cc file that uses them, or the program may fail to link in some build configurations. If declarations and definitions are in different files, including the former should transitively include the latter. Do not move these definitions to separately included header files (-inl.h); this practice was common in the past, but is no longer allowed.

As an exception, a template that is explicitly instantiated for all relevant sets of template arguments, or that is a private implementation detail of a class, is allowed to be defined in the one and only .cc file that instantiates the template.

There are rare cases where a file designed to be included is not self-contained. These are typically intended to be included at unusual locations, such as the middle of another file. They might not use header guards, and might not include their prerequisites. Name such files with the .inc extension. Use sparingly, and prefer self-contained headers when possible.

\subsection{The \#define Guard}

All header files should have \#define guards to prevent multiple inclusion. The format of the symbol name should be <PROJECT>\_<PATH>\_<FILE>\_H\_.

To guarantee uniqueness, they should be based on the full path in a project's source tree. For example, the file foo/src/bar/baz.h in project foo should have the following guard:

\begin{lstlisting}
#ifndef FOO_BAR_BAZ_H_
#define FOO_BAR_BAZ_H_

...

#endif  // FOO_BAR_BAZ_H_
\end{lstlisting}
\subsection{Forward Declarations}

Avoid using forward declarations where possible. Just \#include the headers you need.

A "forward declaration" is a declaration of a class, function, or template without an associated definition.

Forward declarations can save compile time, as \#includes force the compiler to open more files and process more input.
Forward declarations can save on unnecessary recompilation. \#includes can force your code to be recompiled more often, due to unrelated changes in the header.
Forward declarations can hide a dependency, allowing user code to skip necessary recompilation when headers change.
A forward declaration may be broken by subsequent changes to the library. Forward declarations of functions and templates can prevent the header owners from making otherwise-compatible changes to their APIs, such as widening a parameter type, adding a template parameter with a default value, or migrating to a new namespace.
Forward declaring symbols from namespace std:: yields undefined behavior.
It can be difficult to determine whether a forward declaration or a full \#include is needed. Replacing an \#include with a forward declaration can silently change the meaning of code:
\begin{lstlisting}
      // b.h:
      struct B {};
      struct D : B {};

      // good_user.cc:
      #include "b.h"
      void f(B*);
      void f(void*);
      void test(D* x) { f(x); }  // calls f(B*)
\end{lstlisting}

If the \#include was replaced with forward decls for B and D, test() would call f(void*).
Forward declaring multiple symbols from a header can be more verbose than simply \#includeing the header.
Structuring code to enable forward declarations (e.g. using pointer members instead of object members) can make the code slower and more complex.
Try to avoid forward declarations of entities defined in another project.
When using a function declared in a header file, always \#include that header.
When using a class template, prefer to \#include its header file.
Please see Names and Order of Includes for rules about when to \#include a header.

\subsection{Inline Functions}

Define functions inline only when they are small, say, 10 lines or fewer.

You can declare functions in a way that allows the compiler to expand them inline rather than calling them through the usual function call mechanism.

Inlining a function can generate more efficient object code, as long as the inlined function is small. Feel free to inline accessors and mutators, and other short, performance-critical functions.

Overuse of inlining can actually make programs slower. Depending on a function's size, inlining it can cause the code size to increase or decrease. Inlining a very small accessor function will usually decrease code size while inlining a very large function can dramatically increase code size. On modern processors smaller code usually runs faster due to better use of the instruction cache.

A decent rule of thumb is to not inline a function if it is more than 10 lines long. Beware of destructors, which are often longer than they appear because of implicit member- and base-destructor calls!

Another useful rule of thumb: it's typically not cost effective to inline functions with loops or switch statements (unless, in the common case, the loop or switch statement is never executed).

It is important to know that functions are not always inlined even if they are declared as such; for example, virtual and recursive functions are not normally inlined. Usually recursive functions should not be inline. The main reason for making a virtual function inline is to place its definition in the class, either for convenience or to document its behavior, e.g., for accessors and mutators.

\subsection{Names and Order of Includes}

Use standard order for readability and to avoid hidden dependencies: Related header, C library, C++ library, other libraries' .h, your project's .h.

All of a project's header files should be listed as descendants of the project's source directory without use of UNIX directory shortcuts . (the current directory) or .. (the parent directory). For example, google-awesome-project/src/base/logging.h should be included as:

\begin{lstlisting}
#include "base/logging.h"
\end{lstlisting}
In dir/foo.cc or dir/foo\_test.cc, whose main purpose is to implement or test the stuff in dir2/foo2.h, order your includes as follows:
\begin{lstlisting}
dir2/foo2.h.
A blank line
C system files.
C++ system files.
A blank line
Other libraries' .h files.
Your project's .h files.
\end{lstlisting}
Note that any adjacent blank lines should be collapsed.

With the preferred ordering, if dir2/foo2.h omits any necessary includes, the build of dir/foo.cc or dir/foo\_test.cc will break. Thus, this rule ensures that build breaks show up first for the people working on these files, not for innocent people in other packages.

dir/foo.cc and dir2/foo2.h are usually in the same directory (e.g. base/basictypes\_test.cc and base/basictypes.h), but may sometimes be in different directories too.

Note that the C compatibility headers such as stddef.h are essentially interchangeable with their C++ counterparts (cstddef) Either style is acceptable, but prefer consistency with existing code.

Within each section the includes should be ordered alphabetically. Note that older code might not conform to this rule and should be fixed when convenient.

You should include all the headers that define the symbols you rely upon, except in the unusual case of forward declaration. If you rely on symbols from bar.h, don't count on the fact that you included foo.h which (currently) includes bar.h: include bar.h yourself, unless foo.h explicitly demonstrates its intent to provide you the symbols of bar.h. However, any includes present in the related header do not need to be included again in the related cc (i.e., foo.cc can rely on foo.h's includes).

For example, the includes in google-awesome-project/src/foo/internal/fooserver.cc might look like this:
\begin{lstlisting}
#include "foo/server/fooserver.h"

#include <sys/types.h>
#include <unistd.h>
#include <vector>

#include "base/basictypes.h"
#include "base/commandlineflags.h"
#include "foo/server/bar.h"
\end{lstlisting}
Sometimes, system-specific code needs conditional includes. Such code can put conditional includes after other includes. Of course, keep your system-specific code small and localized. Example:

\begin{lstlisting}
#include "foo/public/fooserver.h"

#include "base/port.h"  // For LANG_CXX11.

#ifdef LANG_CXX11
#include <initializer_list>
#endif  // LANG_CXX11
\end{lstlisting}


==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = chern

default: testpdflatex

testlatex:
	latex  ${BASENAME}
	latex  ${BASENAME}
	#bibtex ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}

testpdflatex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	bibtex    ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 



==> Scoping.tex <==
\section{Scoping}
\subsection{Namespaces}

With few exceptions, place code in a namespace. Namespaces should have unique names based on the project name, and possibly its path. Do not use using-directives (e.g. using namespace foo). Do not use inline namespaces. For unnamed namespaces, see Unnamed Namespaces and Static Variables.

Namespaces subdivide the global scope into distinct, named scopes, and so are useful for preventing name collisions in the global scope.

Namespaces provide a method for preventing name conflicts in large programs while allowing most code to use reasonably short names.

For example, if two different projects have a class Foo in the global scope, these symbols may collide at compile time or at runtime. If each project places their code in a namespace, project1::Foo and project2::Foo are now distinct symbols that do not collide, and code within each project's namespace can continue to refer to Foo without the prefix.

Inline namespaces automatically place their names in the enclosing scope. Consider the following snippet, for example:
\begin{lstlisting}
namespace outer {
inline namespace inner {
  void foo();
}  // namespace inner
}  // namespace outer
\end{lstlisting}
The expressions outer::inner::foo() and outer::foo() are interchangeable. Inline namespaces are primarily intended for ABI compatibility across versions.


Namespaces can be confusing, because they complicate the mechanics of figuring out what definition a name refers to.

Inline namespaces, in particular, can be confusing because names aren't actually restricted to the namespace where they are declared. They are only useful as part of some larger versioning policy.

In some contexts, it's necessary to repeatedly refer to symbols by their fully-qualified names. For deeply-nested namespaces, this can add a lot of clutter.

Namespaces should be used as follows:

Follow the rules on Namespace Names.
Terminate namespaces with comments as shown in the given examples.
Namespaces wrap the entire source file after includes, gflags definitions/declarations and forward declarations of classes from other namespaces.

// In the .h file
\begin{lstlisting}
namespace mynamespace {

// All declarations are within the namespace scope.
// Notice the lack of indentation.
class MyClass {
 public:
  ...
  void Foo();
};

}  // namespace mynamespace
\end{lstlisting}
// In the .cc file
\begin{lstlisting}
namespace mynamespace {

// Definition of functions is within scope of the namespace.
void MyClass::Foo() {
  ...
}

}  // namespace mynamespace
\end{lstlisting}
More complex .cc files might have additional details, like flags or using-declarations.

\begin{lstlisting}
#include "a.h"

DEFINE_FLAG(bool, someflag, false, "dummy flag");

namespace mynamespace {

using ::foo::bar;

...code for mynamespace...    // Code goes against the left margin.

}  // namespace mynamespace
\end{lstlisting}
To place generated protocol message code in a namespace, use the package specifier in the .proto file. See Protocol Buffer Packages for details.
Do not declare anything in namespace std, including forward declarations of standard library classes. Declaring entities in namespace std is undefined behavior, i.e., not portable. To declare entities from the standard library, include the appropriate header file.
You may not use a using-directive to make all names from a namespace available.

// Forbidden -- This pollutes the namespace.
using namespace foo;
Do not use Namespace aliases at namespace scope in header files except in explicitly marked internal-only namespaces, because anything imported into a namespace in a header file becomes part of the public API exported by that file.

// Shorten access to some commonly used names in .cc files.
\begin{lstlisting}
namespace baz = ::foo::bar::baz;
// Shorten access to some commonly used names (in a .h file).
namespace librarian {
namespace impl {  // Internal, not part of the API.
namespace sidetable = ::pipeline_diagnostics::sidetable;
}  // namespace impl

inline void my_inline_function() {
  // namespace alias local to a function (or method).
  namespace baz = ::foo::bar::baz;
  ...
}
}  // namespace librarian
\end{lstlisting}
Do not use inline namespaces.
Unnamed Namespaces and Static Variables

When definitions in a .cc file do not need to be referenced outside that file, place them in an unnamed namespace or declare them static. Do not use either of these constructs in .h files.

All declarations can be given internal linkage by placing them in unnamed namespaces. Functions and variables can also be given internal linkage by declaring them static. This means that anything you're declaring can't be accessed from another file. If a different file declares something with the same name, then the two entities are completely independent.

Use of internal linkage in .cc files is encouraged for all code that does not need to be referenced elsewhere. Do not use internal linkage in .h files.

Format unnamed namespaces like named namespaces. In the terminating comment, leave the namespace name empty:

\begin{lstlisting}
namespace {
...
}  // namespace
\end{lstlisting}
\subsection{Nonmember, Static Member, and Global Functions}

Prefer placing nonmember functions in a namespace; use completely global functions rarely. Do not use a class simply to group static functions. Static methods of a class should generally be closely related to instances of the class or the class's static data.

Nonmember and static member functions can be useful in some situations. Putting nonmember functions in a namespace avoids polluting the global namespace.

Nonmember and static member functions may make more sense as members of a new class, especially if they access external resources or have significant dependencies.

Sometimes it is useful to define a function not bound to a class instance. Such a function can be either a static member or a nonmember function. Nonmember functions should not depend on external variables, and should nearly always exist in a namespace. Do not create classes only to group static member functions; this is no different than just giving the function names a common prefix, and such grouping is usually unnecessary anyway.

If you define a nonmember function and it is only needed in its .cc file, use internal linkage to limit its scope.

\subsection{Local Variables}

Place a function's variables in the narrowest scope possible, and initialize variables in the declaration.

C++ allows you to declare variables anywhere in a function. We encourage you to declare them in as local a scope as possible, and as close to the first use as possible. This makes it easier for the reader to find the declaration and see what type the variable is and what it was initialized to. In particular, initialization should be used instead of declaration and assignment, e.g.:

\begin{lstlisting}
int i;
i = f();      // Bad -- initialization separate from declaration.
int j = g();  // Good -- declaration has initialization.
std::vector<int> v;
v.push_back(1);  // Prefer initializing using brace initialization.
v.push_back(2);
std::vector<int> v = {1, 2};  // Good -- v starts initialized.
Variables needed for if, while and for statements should normally be declared within those statements, so that such variables are confined to those scopes. E.g.:
\end{lstlisting}

while (const char* p = strchr(str, '/')) str = p + 1;
There is one caveat: if the variable is an object, its constructor is invoked every time it enters scope and is created, and its destructor is invoked every time it goes out of scope.

// Inefficient implementation:
\begin{lstlisting}
for (int i = 0; i < 1000000; ++i) {
  Foo f;  // My ctor and dtor get called 1000000 times each.
  f.DoSomething(i);
}
\end{lstlisting}
It may be more efficient to declare such a variable used in a loop outside that loop:

\begin{lstlisting}
Foo f;  // My ctor and dtor get called once each.
for (int i = 0; i < 1000000; ++i) {
  f.DoSomething(i);
}
\end{lstlisting}
\subsection{Static and Global Variables}

Objects with static storage duration are forbidden unless they are trivially destructible. Informally this means that the destructor does not do anything, even taking member and base destructors into account. More formally it means that the type has no user-defined or virtual destructor and that all bases and non-static members are trivially destructible. Static function-local variables may use dynamic initialization. Use of dynamic initialization for static class member variables or variables at namespace scope is discouraged, but allowed in limited circumstances; see below for details.

As a rule of thumb: a global variable satisfies these requirements if its declaration, considered in isolation, could be constexpr.

Every object has a storage duration, which correlates with its lifetime. Objects with static storage duration live from the point of their initialization until the end of the program. Such objects appear as variables at namespace scope ("global variables"), as static data members of classes, or as function-local variables that are declared with the static specifier. Function-local static variables are initialized when control first passes through their declaration; all other objects with static storage duration are initialized as part of program start-up. All objects with static storage duration are destroyed at program exit (which happens before unjoined threads are terminated).

Initialization may be dynamic, which means that something non-trivial happens during initialization. (For example, consider a constructor that allocates memory, or a variable that is initialized with the current process ID.) The other kind of initialization is static initialization. The two aren't quite opposites, though: static initialization always happens to objects with static storage duration (initializing the object either to a given constant or to a representation consisting of all bytes set to zero), whereas dynamic initialization happens after that, if required.

Global and static variables are very useful for a large number of applications: named constants, auxiliary data structures internal to some translation unit, command-line flags, logging, registration mechanisms, background infrastructure, etc.

Global and static variables that use dynamic initialization or have non-trivial destructors create complexity that can easily lead to hard-to-find bugs. Dynamic initialization is not ordered across translation units, and neither is destruction (except that destruction happens in reverse order of initialization). When one initialization refers to another variable with static storage duration, it is possible that this causes an object to be accessed before its lifetime has begun (or after its lifetime has ended). Moreover, when a program starts threads that are not joined at exit, those threads may attempt to access objects after their lifetime has ended if their destructor has already run.

Decision on destruction

When destructors are trivial, their execution is not subject to ordering at all (they are effectively not "run"); otherwise we are exposed to the risk of accessing objects after the end of their lifetime. Therefore, we only allow objects with static storage duration if they are trivially destructible. Fundamental types (like pointers and int) are trivially destructible, as are arrays of trivially destructible types. Note that variables marked with constexpr are trivially destructible.

\begin{lstlisting}
const int kNum = 10;  // allowed

struct X { int n; };
const X kX[] = {{1}, {2}, {3}};  // allowed

void foo() {
  static const char* const kMessages[] = {"hello", "world"};  // allowed
}

// allowed: constexpr guarantees trivial destructor
constexpr std::array<int, 3> kArray = {{1, 2, 3}};
// bad: non-trivial destructor
const string kFoo = "foo";

// bad for the same reason, even though kBar is a reference (the
// rule also applies to lifetime-extended temporary objects)
const string& kBar = StrCat("a", "b", "c");

void bar() {
  // bad: non-trivial destructor
  static std::map<int, int> kData = {{1, 0}, {2, 0}, {3, 0}};
}
\end{lstlisting}
Note that references are not objects, and thus they are not subject to the constraints on destructibility. The constraint on dynamic initialization still applies, though. In particular, a function-local static reference of the form static T\& t = *new T; is allowed.

Decision on initialization

Initialization is a more complex topic. This is because we must not only consider whether class constructors execute, but we must also consider the evaluation of the initializer:

\begin{lstlisting}
int n = 5;    // fine
int m = f();  // ? (depends on f)
Foo x;        // ? (depends on Foo::Foo)
Bar y = g();  // ? (depends on g and on Bar::Bar)
\end{lstlisting}
All but the first statement expose us to indeterminate initialization ordering.

The concept we are looking for is called constant initialization in the formal language of the C++ standard. It means that the initializing expression is a constant expression, and if the object is initialized by a constructor call, then the constructor must be specified as constexpr, too:

\begin{lstlisting}
struct Foo { constexpr Foo(int) {} };

int n = 5;  // fine, 5 is a constant expression
Foo x(2);   // fine, 2 is a constant expression and the chosen constructor is constexpr
Foo a[] = { Foo(1), Foo(2), Foo(3) };  // fine
\end{lstlisting}
Constant initialization is always allowed. Constant initialization of static storage duration variables should be marked with constexpr or where possible the ABSL\_CONST\_INIT attribute. Any non-local static storage duration variable that is not so marked should be presumed to have dynamic initialization, and reviewed very carefully.

By contrast, the following initializations are problematic:

\begin{lstlisting}
time_t time(time_t*);      // not constexpr!
int f();                   // not constexpr!
struct Bar { Bar() {} };
\end{lstlisting}
\begin{lstlisting}
time_t m = time(nullptr);  // initializing expression not a constant expression
Foo y(f());                // ditto
Bar b;                     // chosen constructor Bar::Bar() not constexpr
\end{lstlisting}
Dynamic initialization of nonlocal variables is discouraged, and in general it is forbidden. However, we do permit it if no aspect of the program depends on the sequencing of this initialization with respect to all other initializations. Under those restrictions, the ordering of the initialization does not make an observable difference. For example:

\begin{lstlisting}
int p = getpid();  // allowed, as long as no other static variable
                   // uses p in its own initialization
Dynamic initialization of static local variables is allowed (and common).
\end{lstlisting}

\subsection{Common patterns}

Global strings: if you require a global or static string constant, consider using a simple character array, or a char pointer to the first element of a string literal. String literals have static storage duration already and are usually sufficient.
Maps, sets, and other dynamic containers: if you require a static, fixed collection, such as a set to search against or a lookup table, you cannot use the dynamic containers from the standard library as a static variable, since they have non-trivial destructors. Instead, consider a simple array of trivial types, e.g. an array of arrays of ints (for a "map from int to int"), or an array of pairs (e.g. pairs of int and const char*). For small collections, linear search is entirely sufficient (and efficient, due to memory locality). If necessary, keep the collection in sorted order and use a binary search algorithm. If you do really prefer a dynamic container from the standard library, consider using a function-local static pointer, as described below.
Smart pointers (unique\_ptr, shared\_ptr): smart pointers execute cleanup during destruction and are therefore forbidden. Consider whether your use case fits into one of the other patterns described in this section. One simple solution is to use a plain pointer to a dynamically allocated object and never delete it (see last item).
Static variables of custom types: if you require static, constant data of a type that you need to define yourself, give the type a trivial destructor and a constexpr constructor.
If all else fails, you can create an object dynamically and never delete it by binding the pointer to a function-local static pointer variable: static const auto* const impl = new T(args...); (If the initialization is more complex, it can be moved into a function or lambda expression.)
\subsection{thread\_local Variables}

thread\_local variables that aren't declared inside a function must be initialized with a true compile-time constant, and this must be enforced by using the ABSL\_CONST\_INIT attribute. Prefer thread\_local over other ways of defining thread-local data.

Starting with C++11, variables can be declared with the thread\_local specifier:

thread\_local Foo foo = ...;
Such a variable is actually a collection of objects, so that when different threads access it, they are actually accessing different objects. thread\_local variables are much like static storage duration variables in many respects. For instance, they can be declared at namespace scope, inside functions, or as static class members, but not as ordinary class members.

thread\_local variable instances are initialized much like static variables, except that they must be initialized separately for each thread, rather than once at program startup. This means that thread\_local variables declared within a function are safe, but other thread\_local variables are subject to the same initialization-order issues as static variables (and more besides).

thread\_local variable instances are destroyed when their thread terminates, so they do not have the destruction-order issues of static variables.

Thread\-local data is inherently safe from races (because only one thread can ordinarily access it), which makes thread\_local useful for concurrent programming.
thread\_local is the only standard-supported way of creating thread-local data.
Accessing a thread\_local variable may trigger execution of an unpredictable and uncontrollable amount of other code.
thread\_local variables are effectively global variables, and have all the drawbacks of global variables other than lack of thread-safety.
The memory consumed by a thread\_local variable scales with the number of running threads (in the worst case), which can be quite large in a program.
An ordinary class member cannot be thread\_local.
thread\_local may not be as efficient as certain compiler intrinsics.
thread\_local variables inside a function have no safety concerns, so they can be used without restriction. Note that you can use a function-scope thread\_local to simulate a class- or namespace-scope thread\_local by defining a function or static method that exposes it:

\begin{lstlisting}
Foo& MyThreadLocalFoo() {
  thread_local Foo result = ComplicatedInitialization();
  return result;
}
\end{lstlisting}
thread\_local variables at class or namespace scope must be initialized with a true compile-time constant (i.e. they must have no dynamic initialization). To enforce this, thread\_local variables at class or namespace scope must be annotated with ABSL\_CONST\_INIT (or constexpr, but that should be rare):

ABSL\_CONST\_INIT thread\_local Foo foo = ...;
thread\_local should be preferred over other mechanisms for defining thread-local data.


==> tikz-test.tex <==
\usetikzlibrary{arrows}

\tikzstyle{int}=[draw, fill=blue!20, minimum size=2em]
\tikzstyle{init} = [pin edge={to-,thin,black}]

\begin{tikzpicture}[node distance=2.5cm,auto,>=latex']
    \node [int, pin={[init]above:$v_0$}] (a) {$\frac{1}{s}$};
    \node (b) [left of=a,node distance=2cm, coordinate] {a};
    \node [int, pin={[init]above:$p_0$}] (c) [right of=a] {$\frac{1}{s}$};
    \node [coordinate] (end) [right of=c, node distance=2cm]{};
    \path[->] (b) edge node {$a$} (a);
    \path[->] (a) edge node {$v$} (c);
    \draw[->] (c) edge node {$p$} (end) ;
\end{tikzpicture}
